Transforming Slot Schema Induction with Generative Dialogue State Inference

The challenge of defining a slot schema to represent the state of a task-oriented dialogue system is addressed by Slot Schema Induction (SSI), which aims to automatically induce slots from unlabeled dialogue data. Whereas previous approaches induce slots by clustering value spans extracted directly from the dialogue text, we demonstrate the power of discovering slots using a generative approach. By training a model to generate slot names and values that summarize key dialogue information with no prior task knowledge, our SSI method discovers high-quality candidate information for representing dialogue state. These discovered slot-value candidates can be easily clustered into unified slot schemas that align well with human-authored schemas. Experimental comparisons on the MultiWOZ and SGD datasets demonstrate that Generative Dialogue State Inference (GenDSI) outperforms the previous state-of-the-art on multiple aspects of the SSI task.

==> latex/xd_related_work.tex <==

\section{Related Work}
\label{sec:ssi_related_work}

% One of the challenges of applying DST models in practice is specifying a slot schema that defines which slots the DST model should track. In applications where a dialogue model is being integrated into existing software framework, the slot schema is typically specified by hand to match the existing infrastructure such as API call parameters or database schemata. However, in many cases, the external software components interfacing with the dialogue system are under development, and the choice of slots to track is made in tandem with the development of new features. In these cases, a typical developer workflow for creating the slot schema involves manually reviewing unlabeled dialogue data produced by a previous version of the dialogue system or by human-human interaction, and deciding which information is important to track as slots. This workflow is especially prevalent when implementing custom policy changes to the dialogue system behavior, where a developer seeks to control system behavior via programmatic intervention as a response to viewing a poor-quality dialogue produced by their system.

% Slot schema induction (SSI) aims to reduce the cost of manual schema creation by automatically inducing slots from unlabeled dialogue data that are likely to facilitate task completion. The primary challenges of this task are (1) to correctly identify what information in the unlabeled dialogues would be important to track as slot values, and (2) aggregating candidate value information into a consolidated set of useful slot types. As SSI is a relatively recent task with few works, there is yet no standardized task formulation and evaluation method. However, several of the most recent works present similar variants of the following formulation.

% Given a list of dialogues $D$, produce a list of slots $\hat{S} = [\hat{s_1}, \hat{s_2}, ..., \hat{s_n}]$ where each slot $\hat{s_i}$ is a cluster of values $\hat{s_i} = [\hat{v_1}, \hat{v_2}, ..., \hat{v}_{|\hat{s_i}|}]$ corresponding to a gold reference slot $s_i = [v_1, v_2, ..., v_{|s_i|}]$. To evaluate, a mapping $M : \hat{S} \rightarrow S \oplus [\text{none}]$ is constructed by hand or using a semantic similarity estimator to assign each predicted cluster to a gold slot (or to none if no gold slot matches). In this formulation, producing a name for each induced slot is out of scope; the goal is only to find clusters of values that correspond well to gold slots. Given the mapping $M$ from predicted to gold slots, precision, recall, and F1 are calculated to measure the quality of induced slot clusters.

Approaches to slot schema induction follow a two-step pipeline of first extracting value candidates from dialogue text, then clustering dense semantic vector representations of each candidate to produce slot clusters. \citet{hudecek_discovering_2021, wu_semi-supervised_2022, qiu_structure_2022} leverage tagging models trained on other tasks such as Semantic Role Labeling (SRL) or Named Entity Recognition (NER) to identify a set of value candidates from spans in the unlabelled dialogue data. Then, each candidate value is embedded into a dense vector representation using an encoder model such as BERT \cite{devlin-etal-2019-bert}. Finally, a clustering algorithm is used to induce the slot types from the value candidate span representations, often in conjunction with a filtering step to eliminate noisy candidate values. \citet{hudecek_discovering_2021} use a simple cosine-similarity-based threshold to filter value candidates and merge them into clusters. \citet{wu_semi-supervised_2022} use an iterative, self-supervised method to alternate between fine-tuning the candidate value tagging model and cluster candidates, where the tagger learns to select candidates near the centroid of induced clusters. Instead of using NER and SRL models to identify value spans, \cite{qiu_structure_2022} train a domain-general value tagger to identify value candidates, then use out-of-the-box clustering algorithms such as K-Means\footnote{Incurs the limitation of requiring the number of induced slot clusters $K$ to be specified ahead of time.} to induce slot types. One fully unsupervised approach for slot schema induction by \citet{yu_unsupervised_2022} uses a PLM attention distributions between tokens in a dialogue turn to infer the syntactic structure of the turn, and treat constituents as candidate values. Three clustering steps are then followed to obtain a cluster hierarchy, where different encodings of the span candidates are clustered at each step using HDBSCAN \cite{mcinnes_hdbscan_2017}. 

Overall, the SoTA in slot schema induction is encouraging but not practical. The reported recall of predicting slot clusters that match gold slot clusters is quite high with the SoTA achieving 94\% recall on MultiWOZ. However, most slot induction methods induce a number of slots that is about 10x the number of gold slots in a given domain, which still requires a large human effort to manually name and consolidate the clusters into a usable slot schema. Furthermore, a limitation to all previous work in this area is that value candidates are always extracted spans from the orignial dialogue text. This limits the ability of these approaches to induce abstractive slots, whose values rarely appear in the dialogue directly but are nevertheless critical to tracking the dialogue state. 

==> latex/ya_dsgi_example.tex <==

% \section{DSG-I Example}
% \label{appx:ssi_dsgi_example}

% Table \ref{tab:dsgi-example-induction} presents a random sample of all clusters induced by \texttt{IGS} that correspond to a \texttt{Hotel} slot in the gold slot schema, as judged by a human matcher.

% \newcommand{\dashrule}[1][black]{%
%   \color{#1}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}\xleaders\hbox{\rule{4pt}{0pt}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}}\hfill\kern0pt%
% }

% \begin{table*}[htbp]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{p{0.90\textwidth}l}
%         \midrule
%         \multicolumn{2}{c}{\bf Book Stay} \\
%         \midrule
%         A: thank you . i would also like entertainment options in the same area as you booked the hotel . & \texttt{num nights: 3} \\
%         A: yes , i need it for 2 people and 5 nights starting from tuesday . i would also like the reference number . & \texttt{num nights: 5} \\
%         A: can you book it for 4 people for 4 nights starting on thursday ? & \texttt{num nights: 4} \\
%         \multicolumn{2}{@{}c@{}}{\makebox[1.4\columnwidth]{\dashrule[black]}} \\ %[-\jot] \\
%         A: yes , i would like to book 5 nights at the leverton house . & \texttt{stay duration: 5 nights} \\
%         A: book it for thursday night , 3 nights , and 4 people . thank you ! & \texttt{duration: 3 nights} \\
%         A: it s just 1 night for 4 people . & \texttt{stay duration: 1 night} \\
%         \midrule
%         \multicolumn{2}{c}{\bf Internet} \\
%         \midrule
%         A: i do not have an area preference but it needs to have free wifi and parking at a moderate price . & \texttt{free wifi: Yes} \\ \\
%         B: hobsons house is a moderate -ly priced , 3 star guest house in the west . it offers free internet and parking . would you like me to book this for you ? & \multirow{3}{*}{\texttt{free internet: yes}} \\
%         A: great , can i please have the address and phone number ? & \\ \\
%         B: the cambridge belfry also include -s free wifi . i would be more than happy to make your reservations , would you like to do so ? & \multirow{3}{*}{\texttt{wifi situation: Free}} \\
%         A: yes make reservations for 6 people for 5 nights & \\
%         \midrule
%         \multicolumn{2}{c}{\bf Parking} \\
%         \midrule
%         A: please pick 1 that has free parking . & \texttt{free parking: 1} \\
%         A: i would prefer something with 2 stars , and i need free parking as well . & \texttt{parking requirement: free parking} \\
%         A: i am looking for someplace to stay . i would like something expensive , and i do not need parking . & \texttt{parking needed: No parking needed}
%         \\
%         \midrule
%         \multicolumn{2}{c}{\bf Stars} \\
%         \midrule
%         A: i am flexible about cost , i would prefer free wifi and a 4 star rating though . & \texttt{4 star rating: Yes} \\ \\
%         B: the ashley hotel and the lovell lodge are both in the north and are in the moderate price range with 2 stars . & \multirow{3}{*}{\texttt{star rating: 2 stars}} \\
%         A: will you book it for a party of 7 . 5 days beginning friday . & \\ \\
%         A: the star preference does not matter . i'll take the 4 star . & \texttt{star preference: 4} \\
%         \multicolumn{2}{@{}c@{}}{\makebox[1.4\columnwidth]{\dashrule[black]}} \\ %[-\jot] \\
%         A: yes , i am also looking for a 3 star hotel located in the same area as the restaurant . & \texttt{hotel type: 3 star} \\
%         A: the hotel should include free parking and should have a star of 3 . & \texttt{hotel star rating: 3} \\
%         A: i am looking for a 4 star hotel in the south . & \texttt{hotel rating: 4 star} \\
%         \midrule
%         \multicolumn{2}{c}{\bf Book Day} \\
%         \midrule
%         A: yes , please recommend 1 that can accommodate 8 people for 2 nights starting on thursday & \texttt{start date: Thursday} \\
%         A: 4 people for 2 nights starting sunday , please ! & \texttt{start date: Sunday} \\
%         A: great ! i would like to book rooms for 5 people for 4 nights starting friday . & \texttt{start date: friday} \\
%         \midrule
%         \multicolumn{2}{c}{\bf Area} \\
%         \midrule
%         A: hi , i am looking for a moderate -ly priced hotel in the east . & \texttt{hotel location: East} \\
%         A: i am looking for a hotel with free parking in the north . & \texttt{hotel location: North} \\
%         A: i need a hotel in the south with free wifi . & \texttt{hotel location: South} \\
%         \midrule
%         \multicolumn{2}{c}{\bf Price Range} \\
%         \midrule
%         A: thank you , i am also looking for a hotel in the east that has free parking for my car . i'll need the hotel to be cheap with wifi & \texttt{hotel budget: Cheap} \\
%         A: hi , i am looking for a moderate -ly priced hotel in the east . & \texttt{hotel type: Moderate -ly priced} \\
%         A: hmm , well how about checking for a hotel instead that is expensive with free parking and wifi ? & \texttt{hotel type: Expensive} \\
%         \midrule
%         \multicolumn{2}{c}{\bf Type} \\
%         \midrule
%         A: thanks i am also needing to book at a guest house for 6 for 5 nights starting on sunday & \texttt{room type: Guest house} \\
%         A: let s go with a hotel . i would actually like it to have free internet and parking , if possible . & \texttt{hotel or guest house: Hotel} \\
%         A: i am looking for a place to stay . ideally , it will be a guest house and have a 4 star rating . & \texttt{accommodation type: Guest house}
%     \end{tabular}
%     }
%     \caption{Examples of DSG-I results mapping to the gold \texttt{Hotel} slots of MultiWOZ. Dashed lines separate individual DSG-I clusters that map to the same gold slot.}
%     \label{tab:dsgi-example-induction}
% \end{table*}
